Ambiguities in Partial Wave Analysis of Two Spinless Meson Photoproduction

We describe the formalism to analyze the mathematical ambiguities arising in partial-wave analysis of two spinless mesons produced with a linearly polarized photon beam. We show that partial waves are uniquely defined when all accessible observables are considered, for a wave set which includes $S$ and $D$ waves. The inclusion of higher partial waves does not affect our results, and we conclude that there are no mathematical ambiguities in partial-wave analysis of two mesons produced with a linearly polarized photon beam. We present Monte Carlo simulations to illustrate our results.

==> logos/JPAC-colors.tex <==
\definecolor{jpac-blue}{RGB}{ 31,119,180}%  hex = #1F77B4
\definecolor{jpac-red}{RGB}{214,39, 40}%  hex = #D61D28
\definecolor{jpac-green}{RGB}{ 44,160, 44}%  hex = #2CA02C
\definecolor{jpac-orange}{RGB}{255,127, 14}%  hex = #FF7F0E
\definecolor{jpac-purple}{RGB}{148,103,189}%  hex = #9467BD
\definecolor{jpac-brown}{RGB}{140, 86, 75}%  hex = #8C564B
\definecolor{jpac-pink}{RGB}{227,119,194}%  hex = #E377C2
\definecolor{jpac-gold}{RGB}{188,189, 34}%  hex = #BCBD22
\definecolor{jpac-aqua}{RGB}{ 23,190,207}%  hex = #17BECF
\definecolor{jpac-grey}{RGB}{127,127,127}%  hex = #7F7F7F

